TAPEX: Table Pre-training via Learning a Neural SQL Executor

Recent progress in language model pre-training has achieved a great success via leveraging large-scale unstructured textual data. However, it is still a challenge to apply pre-training on structured tabular data due to the absence of large-scale high-quality tabular data. In this paper, we propose TAPEX to show that table pre-training can be achieved by learning a neural SQL executor over a synthetic corpus, which is obtained by automatically synthesizing executable SQL queries and their execution outputs. TAPEX addresses the data scarcity challenge via guiding the language model to mimic a SQL executor on the diverse, large-scale and high-quality synthetic corpus. We evaluate TAPEX on four benchmark datasets. Experimental results demonstrate that TAPEX outperforms previous table pre-training approaches by a large margin and achieves new state-of-the-art results on all of them. This includes the improvements on the weakly-supervised WikiSQL denotation accuracy to 89.5% (+2.3%), the WikiTableQuestions denotation accuracy to 57.5% (+4.8%), the SQA denotation accuracy to 74.5% (+3.5%), and the TabFact accuracy to 84.2% (+3.2%). To our knowledge, this is the first work to exploit table pre-training via synthetic executable programs and to achieve new state-of-the-art results on various downstream tasks. Our code can be found at https://github.com/microsoft/Table-Pretraining.

==> Camera-Ready-ICLR 2022-Tapex/0_abstract.tex <==


Recent progress in language model pre-training has achieved a great success via leveraging large-scale unstructured textual data. However, it is still a challenge to apply pre-training on structured tabular data due to the absence of large-scale high-quality tabular data.
In this paper, we propose \ourexp to show that table pre-training can be achieved by learning a neural SQL executor over a synthetic corpus, which is obtained by automatically synthesizing executable SQL queries and their execution outputs.
\ourexp addresses the data scarcity challenge via guiding the language model to mimic a SQL executor on the diverse, large-scale and high-quality synthetic corpus.
We evaluate \ourexp on four benchmark datasets. 
Experimental results demonstrate that \ourexp outperforms previous table pre-training approaches by a large margin and achieves new state-of-the-art results on all of them.
This includes improvements on the weakly-supervised WikiSQL denotation accuracy to $\mathbf{89.5}\%$ ($+2.3\%$), the WikiTableQuestions denotation accuracy to $\mathbf{57.5}\%$ ($+4.8\%$), the SQA denotation accuracy to $\mathbf{74.5}\%$ ($+3.5\%$), and the TabFact accuracy to $\mathbf{84.2\%}$ ($+3.2\%$).
To our knowledge, this is the first work to exploit table pre-training via synthetic executable programs and to achieve new state-of-the-art results on various downstream tasks.
Our code can be found at \url{https://github.com/microsoft/Table-Pretraining}.

==> Camera-Ready-ICLR 2022-Tapex/10_ethics_statement.tex <==
\section*{Ethics Statement}

In this work, we present a novel pre-training approach for tabular data, which approximates the structural reasoning process of formal languages over tables to achieve efficient table pre-training.
Different from previous works which employ web crawling to construct a large-scale NL-table corpus for pre-training, our pre-training corpus is synthesized via sampling SQL queries and their execution results on public tables.
Compared with previous works, our pre-training corpus is more controllable with high-quality.
For example, compared with \tabert which crawls $26$ million noisy tables from the Web, our approach adopts $1,500$ high-quality tables from public datasets, which greatly alleviates the potential privacy and bias issues raised by web crawling.
We evaluate our approach on two fundamental table-related tasks: table-based question answering and table-based fact verification.
The former enables non-expert users to query databases without learning programming languages, while the latter helps users to verify whether a textual hypothesis is valid based on given tabular evidence.
Experimental results on four well-known benchmark datasets show that our approach achieves new state-of-the-art results on all of them, especially in the low data regime.

==> Camera-Ready-ICLR 2022-Tapex/1_introduction.tex <==

\section{Introduction}\label{sec:intro}

Pre-trained language models (LMs) such as BERT \citep{devlin-etal-2019-bert} and BART \citep{lewis-etal-2020-bart} have hit a success on a range of free-form natural language (NL) tasks.
By learning from a large amount of unstructured textual data, these models have demonstrated surprising capabilities in understanding NL sentences.
Inspired by this huge success, researchers have attempted to extend pre-training to structured tabular data \citep{herzig-etal-2020-tapas,yin-etal-2020-tabert,Yu2020GraPPaGP,wang2021tuta,DBLP:journals/pvldb/DengSL0020,deng-etal-2021-structure,DBLP:conf/aaai/ShiNWZLWSX21}.
However, different from free-form NL sentences, tabular data often contains rich and meaningful structural information, for which existing pre-training approaches designed for unstructured data are not well suited.

To apply pre-training techniques on structured tabular data, there exist two key challenges: (i) where to obtain a large-scale pre-training corpus with high quality, and (ii) 
how to design an efficient pre-training task for table pre-training.
For the first challenge, existing works generally collect parallel data including NL sentences and tables as the pre-training corpus, since downstream tasks often involve a joint reasoning over both free-form NL sentences and tables.
They either crawled tables and their surrounding NL sentences from the Web \citep{herzig-etal-2020-tapas,yin-etal-2020-tabert,deng-etal-2021-structure}, or synthesized NL sentences on available tables \citep{Yu2020GraPPaGP,DBLP:conf/aaai/ShiNWZLWSX21}.
However, as pointed by \citet{yin-etal-2020-tabert}, the raw data mined from the Web is extremely noisy and requires complicated heuristics to clean.
Conversely, the synthesis method is easier to control the data quality, but it usually requires experts to write hundreds of templates, which is both costly and often lacking  diversity.
Regarding the pre-training task, existing works often employ different variants of Masked Language Modeling (MLM) \citep{devlin-etal-2019-bert} to guide LMs to learn better representations of tabular data.
For example, \tapas~\citep{herzig-etal-2020-tapas} used MLM with whole word masking, and \tabert~\citep{yin-etal-2020-tabert} proposed Masked Column Prediction (MCP) to encourage the model to recover the names and data types of masked columns.
Despite their success, they still largely treat tabular data as a structural format of text, which leads to the need of an extremely large corpus for their table pre-training.
All of these hinder the progress of table pre-training.

In this paper, we present a novel execution-centric table pre-training approach \ourexp (\textbf{T\textsc{a}}ble \textbf{P}re-training via \textbf{E\textsc{x}}ecution).
It addresses the above challenges and achieves efficient table pre-training via approximating the structural reasoning process of formal languages over tables.
The structural reasoning process is associated with the executability of tables, i.e., tables are inherently capable of supporting various reasoning operations (e.g., summing over a column in the table).
In particular, \ourexp approximates the structural reasoning process of SQL queries by pre-training LMs to mimic the behavior of a SQL execution engine on tables. 
As shown in~\reffig{fig:model_intro}, by sampling executable SQL queries over tables, \ourexp first synthesizes a large-scale pre-training corpus. 
Then it continues pre-training a language model to output the execution results of these SQL queries, which are obtained from the SQL execution engine.
Since the diversity of SQL queries can be systematically guaranteed, we can easily synthesize a diverse, large-scale, and high-quality pre-training corpus.
Our key insight is that if a language model can be pre-trained to faithfully ``execute'' SQL queries and produce correct results, it should have a deep understanding of tables.
Thus, the execution pre-training task could be more efficient in understanding tables and reasoning over tables.
To our knowledge, \ourexp is the first one to explore table pre-training via synthetic executable programs.

\ourexp is conceptually simple and easy to implement.
In this paper, we regard the pre-training as a sequence generation task and employ an encoder-decoder model.
Specifically, we employ the pre-trained encoder-decoder language model BART~\citep{lewis-etal-2020-bart} as the backbone.
Furthermore, we examine the effectiveness of \ourexp via two fundamental downstream tasks: table-based question answering (TableQA) and table-based fact verification (TableFV).
To enable fine-tuning of downstream tasks to take full advantage of \ourexp, we reformulate these tasks using the encoder-decoder sequence generation paradigm.
We evaluate \ours using four well-known benchmark datasets.
Experimental results clearly demonstrate that \ours can bring significant and consistent improvements on these datasets.
For example, \ourexp obtains an absolute improvement of $19.5\%$ over BART in the \wtq dataset.
Furthermore, \ourexp yields strong results even with a small pre-training corpus, demonstrating its high efficiency.
Finally, \ourexp achieves new state-of-the-art results on all experimental benchmarks, outperforming previous approaches by a large margin, including complicated table pre-training approaches with several heuristics in data processing.
We will make our code, model, and data publicly available to facilitate future research.

\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/intro_model_13.pdf}
    \caption{The schematic overview of our method. For the sake of brevity, the table content in the input is simplified with the symbol $\mathtt{[Table]}$.}
    \label{fig:model_intro}
\end{figure}


==> Camera-Ready-ICLR 2022-Tapex/2_model.tex <==
\section{Fine-Tuning on Downstream Tasks}

Before diving into the details of our proposed table pre-training, we start by describing how to tackle downstream task fine-tuning with the encoder-decoder sequence generation paradigm.
In this section, we first present the background of two fundamental table related downstream tasks: table-based question answering (TableQA) and table-based fact verification (TableFV).
Then we elaborate on our generative fine-tuning method in detail.

\subsection{Downstream Task Formulation}

As mentioned in \refsec{sec:intro}, downstream tasks always involve joint reasoning over free-form NL sentences and tables.
Therefore, examples of downstream tasks generally contain an NL sentence $\mathbf{x}$ and a (semi-)structured table $T$ as the model input.
Each NL sentence consists of $K$ tokens as $\mathbf{x}=x_1,x_2,{\cdots},x_K$, while each table $T$ consists of $M$ rows $\{r_i\}_{i=1}^M$, in which each row $r_i$ contains $N$ cell values $\{s_{{\langle }i,j{\rangle}}\}_{j=1}^{N}$.
Each cell $s_{{\langle }i,j{\rangle}}$ includes a list of tokens and corresponds to a table header $c_j$.
As for the output, there are variations among different tasks.
In this paper, we focus on TableQA and TableFV.
TableQA aims to retrieve table content to answer the user's question, and thus its output is either a list of cell values or number(s) calculated over the selected table region by aggregation functions (e.g., \texttt{SUM}).
It is worth noting that for semi-structured tables, the answer may not be exactly table cell values, but their normalized forms (e.g., from \texttt{2k} to \texttt{2,000}), which makes downstream tasks more challenging \citep{oguz2020unified}.
As for TableFV, the output is a binary decision \textit{entailed} or \textit{refused}, indicating whether the NL sentence follows the fact indicated by the table.


\subsection{Generative Fine-Tuning}\label{sec:getar}

In this section, we present a generative approach for downstream task fine-tuning.
Unlike previous works, we model both TableQA and TableFV as sequence generation tasks and leverage generative LMs to generate the output autoregressively.
Taking TableQA as an example, given an NL question, our method generates the answer by decoding it in a word-by-word fashion.

\textbf{Architecture}\;\;
Our method theoretically applies for any LM as long as it can generate sequence, such as GPT3 \citep{NEURIPS2020_1457c0d6} and UniLM \citep{Bao2020UniLMv2PL}.
In our experiments, we implemented our method based on BART \citep{lewis-etal-2020-bart}, a widely used pre-trained encoder-decoder model.
BART follows a standard sequence-to-sequence Transformer architecture \citep{Vaswani2017AttentionIA}, with modifying ReLU activation functions to GeLU.
It is pre-trained via corrupting sentences (i.e., randomly sampling length-variable spans and masking each one with a single \texttt{[MASK]} token) and then optimizing a reconstruction loss.
As for the number of layers, we employ the $\text{BART}_{\rm Large}$ configuration in our experiments, i.e., 12 layers are used in both the encoder and the decoder.

\textbf{Model Input}\;\;
As illustrated in~\reffig{fig:model_finetune}, the input contains an NL sentence and its corresponding table.
Encoding the NL sentence is relatively straightforward, while encoding the table is non-trivial since it exhibits underlying structures.
In practice, we flatten the table into a sequence so that it can be fed directly into the model.
By inserting several special tokens to indicate the table boundaries, a flattened table can be represented as $T^*=\texttt{\small [HEAD]},c_1,{\cdots},c_N,\texttt{\small [ROW]},1,r_1,\texttt{\small [ROW]},2,r_2,{\cdots},r_M$.
Here \texttt{\small [HEAD]} and \texttt{\small [ROW]} are special tokens indicating the region of table headers and rows respectively, and the number after \texttt{\small [ROW]} is used to indicate the row index.
Notably, we also separate headers or cells in different columns using a vertical bar $|$ .
Finally, we prefix the flattened table $T^*$ with the NL sentence $\mathbf{x}$ and feed them into the model encoder.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/model_finetune_2.pdf}
    \caption{The illustration of the fine-tuning procedure in our method. During fine-tuning, we feed the concatenation of an NL sentence and its corresponding table taken from the downstream task to the model, and train it to output the answer (e.g., ``Marisela Moreno Montero'').}
    \label{fig:model_finetune}
\end{figure*}


\textbf{Model Output}\;\;
With attending on the encoder, the decoder is responsible for modeling the outputs of both TableQA and TableFV.
For TableQA, the output is the concatenation of the answer(s) separated by commas, and the decoder generates it autoregressively.
In this way, our model can readily support (almost) all operators and their compositions in TableQA.
For TableFV, as BART does for sequence classification tasks \citep{lewis-etal-2020-bart}, the same input is fed into both the encoder and decoder, and a binary classifier upon the hidden state of the last token in the decoder is used for the output.
Notably, our method can be easily extended to other table related tasks in a similar way.

\textbf{Fine-Tuning Strategy}\;\;
Since our approach can perform various downstream tasks on the same architecture, it can easily perform multi-task learning.
Therefore, we explore two ways of fine-tuning, one for vanilla fine-tuning and the other for multi-task fine-tuning.
The former is to fine-tune the model on each individual downstream task.
The latter is inspired by \tapas~\citep{herzig-etal-2020-tapas} and T5~\citep{raffel2020exploring}, which first fine-tunes the model on related or similar intermediate downstream tasks and then continues to fine-tune it on the target downstream task.

\textbf{Discussion}\;\;
Our approach comes with several advantages: 
(i) \textit{Flexibility}: due to the powerful expressiveness of encoder-decoder models, our approach can readily adapt to (almost) any kind of output.
(ii) \textit{Conveniency}: our approach does not require any modification (e.g., table-specific masking) on pre-trained LMs, and can be trained in an end-to-end manner.
(iii) \textit{Transferability}: since we formulate downstream tasks as sequence generation tasks, which allows different tasks to share the same training protocol, it is easy to perform multi-task fine-tuning for our approach.



==> Camera-Ready-ICLR 2022-Tapex/3_pretraining.tex <==

\section{Table Pre-training via Execution}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/model_pretrain_15.pdf}
    \caption{The illustration of the pre-training procedure in our method. During pre-training, we feed the concatenation of a sampled SQL query and a sampled table to the model, and train it to output the corresponding execution result (e.g., ``Pairs'').}
    \label{fig:model_pretrain}
\end{figure*}

As mentioned in~\refsec{sec:intro}, \ourexp achieves efficient table pre-training by training LMs to mimic the behavior of a SQL execution engine.
In this section, we illustrate how to conduct table pre-training from two aspects: the pre-training task and the pre-training corpus.

\subsection{Pre-training Task}

Following the MLM task in NL pre-training, existing works usually use reconstruction tasks for table pre-training.
They generally take corrupted tables and NL sentences as input and try to recover the corrupted parts, in order to strengthen the linking between NL sentences and tables.
While these pre-training tasks perform well, they tend to be less efficient since they usually require an extremely large pre-training corpus.

To design efficient tasks for table pre-training, we argue that the key lies in the executability of tables.
That is to say, structured tables enable us to perform discrete operations on them via programming languages such as SQL queries, while unstructured text does not.
Taking this into account, \ours adopts SQL execution as the \textbf{only} pre-training task.
As illustrated in \reffig{fig:model_pretrain}, the pre-training of \ourexp is similar to the procedure of the above generative fine-tuning.
Given an executable SQL query and a table $T$, \ours first concatenates the SQL query and the flattened table $T^*$ to feed into the model encoder.
Then it obtains the query's execution result through an off-the-shelf SQL executor (e.g., MySQL) to serve as the supervision for the model decoder.
Intuitively, the pre-training procedure is to encourage a language model to be a neural SQL executor.
We believe that if a language model can be trained to faithfully ``execute'' SQL queries and produce correct results, then it should have a deep understanding of tables.

\subsection{Pre-training Corpus}

Synthesizing the pre-training corpus is very important for table pre-training.
Generally, there are two key factors: the table source and the SQL query sampling strategy.

\textbf{Table Source}\;\;
Following previous work by~\citet{yin-etal-2020-tabert}, we choose publicly available semi-structured tables as the table source.
However, rather than requiring millions of raw tables in~\citep{yin-etal-2020-tabert}, \ours works well even with only a few thousand tables.
Therefore, instead of fetching noisy tables from the Web and then heuristically filtering them, we pick high-quality tables right from existing public datasets.
Concretely, we randomly select nearly $1,500$ tables from the training set of \wtq~\citep{pasupat2015compositional} as the table source for our pre-training corpus.
Notice that there is no overlap between the tables used in our pre-training and the tables used in the dev and test sets of all downstream tasks, so there is no data leakage problem.

\textbf{Query Sampling}\;\;
Regarding the sampling of diverse SQL queries, there are various choices in the literature.
We can either sample SQL queries according to a probabilistic context-free grammar \citep{wang-etal-2021-learning-synthesize}, or instantiate SQL templates over different tables \citep{zhong-etal-2020-grounded}.
In our experiments, we follow the latter, where SQL templates are automatically extracted from the \textsc{Squall} dataset \citep{shi-etal-2020-potential}.
An example SQL template is: \texttt{\small SELECT num$_1$ WHERE text$_1$ = val$_1$}, where \texttt{\small num$_1$} and \texttt{\small text$_1$} correspond to a numeric column and a text column respectively, and \texttt{\small val$_1$} refers to one of the cell values with respect to the column \texttt{\small text$_1$}.
Given a SQL template, at each instantiation, we uniformly sample headers and cell values from a sampled table to fill the template, forming a concrete SQL query.
Notably, SQL queries that execute with empty results are discarded, because empty results do not reflect much information about the executability of tables.
This way, we can obtain a large-scale pre-training corpus with high quality.

==> Camera-Ready-ICLR 2022-Tapex/5_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

In this section, we evaluate \ourexp on different downstream tasks to verify its effectiveness.

\begin{table}[t]
\small
\begin{minipage}{0.52\linewidth}
\centering
\scalebox{1.0}{
\begin{tabular}{lll}
\toprule
  \textbf{Model} & \textbf{Dev} & \textbf{Test} \\
  \toprule
\multicolumn{3}{c}{\textit{Previous Systems}} \\
\citet{Guo2019UsingDR} & $61.1$ & $61.0$ \\
\citet{liang18mapo}       &  $71.8$  & $72.4$ \\
\citet{Agarwal2019LearningTG}  &  $74.9$  & $74.8$ \\
\citet{wang-etal-2019-learning}     &  $79.4$  & $79.3$ \\ 
\multicolumn{3}{c}{\textit{Pre-trained Language Models}} \\
\citet{min-etal-2019-discrete}     &  $84.4$  & $83.9$ \\
~~~~~~\textit{w.} Execution-Guided Decoding & $87.4$ & $87.2$  \\
\citet{herzig-etal-2020-tapas} & $85.1$ & $83.6$ \\
\citet{Yu2020GraPPaGP} & $85.9$ & $84.7$ \\
\midrule
BART & $87.3$ &  $85.8$ \\
\ours & $\mathbf{89.2}$ & $\mathbf{89.5}$  \\
\bottomrule
\end{tabular}
}
\caption{Denotation accuracies on \wikisql. \textit{Execution-Guided Decoding} is proposed to leverage execution results of SQL queries during inference~\citep{Wang2018RobustTG}.}
\label{tab:wikisql_results}
\end{minipage}
\hspace{2pt}
\begin{minipage}{0.45\linewidth}
\centering
\scalebox{1.0}{
\begin{tabular}{@{}lll@{}}
\toprule
 \textbf{Model} & \textbf{Dev} & \textbf{Test} \\
\midrule
\multicolumn{3}{c}{\textit{Previous Systems}} \\
\citet{pasupat2015compositional}  & $37.0$ & $37.1$ \\
\citet{DBLP:journals/corr/NeelakantanLS15} & $34.1$ & $34.2$ \\
\citet{zhang-etal-2017-macro}  & $40.6$ & $43.7$ \\
\citet{liang18mapo}  & $42.7$ & $43.8$ \\ 
\citet{Dasigi2019IterativeSF} & $43.1$ & $44.3$ \\
\citet{Agarwal2019LearningTG} & $43.2$ & $44.1$ \\ 
\citet{wang-etal-2019-learning} & $43.7$ & $44.5$ \\
\multicolumn{3}{c}{\textit{Pre-trained Language Models}} \\
\citet{herzig-etal-2020-tapas} & ~~~{--} & $48.8$ \\
\citet{yin-etal-2020-tabert} & $53.0$ & $52.3$ \\
\citet{Yu2020GraPPaGP} & $51.9$ & $52.7$ \\
\midrule
BART & $37.2$ & $38.0$ \\
\ours & $\mathbf{57.0}$\; & $\mathbf{57.5}$\; \\
\bottomrule
\end{tabular}
}
\caption{Denotation accuracies on \wtq.}
\label{tab:wtq_results}
\end{minipage}
\end{table}

\paragraph{Dataset and Evaluation} We evaluate the performance of our approach on weakly-supervised WikiSQL (\wikisql)~\citep{zhongSeq2SQL2017}, \wtq~\citep{pasupat2015compositional}, \sqa~\citep{iyyer2017search}, and \tabfact~\citep{chen2019tabfact}.
Compared to \wikisql, which only requires filtering and optionally aggregating on table cell values, \wtq requires more complicated reasoning capabilities.
\sqa is a conversational benchmark, which requires our approach to model the conversational context.
Datset details can be found in~\refapp{appendix:example}.
For TableQA datasets, the evaluation metric is denotation accuracy, which checks whether the predicted answer(s) is equal to the ground-truth answer(s).
It is worth noting that we evaluate our approach on \wikisql with answer annotations provided by \tapas~\citep{herzig-etal-2020-tapas}, since nearly $2\%$ of answers obtained from the official evaluation script are incorrect.
For \tabfact, the evaluation metric is accuracy, which is calculated using the percentage of correct prediction.


\begin{table}[t]
\small
\centering
\begin{tabular}{llllll}
\toprule
\textbf{Model} & \textbf{ALL} & \textbf{SEQ} & $\mathbf{Q}_1$ & $\mathbf{Q}_2$ & $\mathbf{Q}_3$ \\
\midrule
\multicolumn{6}{c}{\textit{Previous Systems}} \\
  \citet{pasupat2015compositional}       &  $33.2$  & ~~$7.7$ & $51.4$ & $22.2$ & $22.3$ \\
  \citet{DBLP:conf/iclr/NeelakantanLAMA17}       &  $40.2$  & $11.8$ & $60.0$ & $35.9$ & $25.5$ \\
  \citet{iyyer2017search}          &  $44.7$  & $12.8$ & $70.4$ & $41.1$ & $23.6$ \\
  \citet{liu-etal-2019-split} & ~~{--} & ~~{--} & $70.9$ & $39.5$ & ~~{--} \\
  \citet{Sun2019KnowledgeAwareCS}     &  $45.6$  & $13.2$ & $70.3$ & $42.6$ & $24.8$ \\ 
  \citet{mueller-etal-2019-answering}     &  $55.1$  & $28.1$ & $67.2$ & $52.7$ & $46.8$ \\
  \multicolumn{6}{c}{\textit{Pre-trained Language Models}} \\
  \citet{Yu2021SCoRePF} & $65.4$ & $38.5$ & $78.4$ & $65.3$ & $55.1$ \\
\citet{herzig-etal-2020-tapas} & $67.2$ & $40.4$ & $78.2$ & $66.0$ & $59.7$ \\
\citet{eisenschlos-etal-2020-understanding} & $71.0$ & $44.8$  & $\mathbf{80.9}$ & $70.6$ & $64.0$ \\
\midrule
BART & $58.6$ & $27.8$ & $65.3$ & $54.1$ & $57.0$ \\
\ours & $\mathbf{74.5}$ & $\mathbf{48.4}$ & $76.2$ & $\mathbf{71.9}$ & $\mathbf{76.9}$ \\\bottomrule
\end{tabular}
\caption{Denotation accuracies on \sqa test set. ALL is the denotation accuracy over all sentences, SEQ the denotation accuracy over all conversations, and $\mathbf{Q}_i$ the denotation accuracy of the i-th sentence in a conversation.}
\label{tab:sqa_results}
\end{table}

\paragraph{Implementation Details}
We implement our approach based on fairseq~\citep{ott2019fairseq}.
During pre-training, we synthesize up to $5$ million pairs of SQL queries and their execution results for \ours.
In the following, unless specified explicitly, all the experimental results are by default evaluated under the $5$ million setting.
Our pre-training procedure runs up to $50,000$ steps with a batch size of $256$.
It takes about $36$ hours on $8$ Tesla V100 GPUs to finish the pre-training.
The best pre-training checkpoint is selected based on the loss on the validation set.
For all downstream datasets, the fine-tuning procedure runs up to $20,000$ steps with a batch size of $128$.
For both pre-training and fine-tuning, the learning rate is $3{\times}{10}^{-5}$.

\subsection{Main Results}

\reftab{tab:wikisql_results}, \reftab{tab:wtq_results}, \reftab{tab:sqa_results} and \reftab{tab:tabfact_results} summarize the experimental results of various models on \wikisql, \wtq, \sqa and \tabfact respectively.
For both dev and test sets of all datasets, we report the median performance of our approach for five random runs.

\textbf{\wikisql}\;\;
As shown in \reftab{tab:wikisql_results}, \ours outperforms all the baselines by a large margin.
On the test set of \wikisql, \ourexp registers a denotation accuracy of $89.5\%$, which is $3.7\%$ higher than BART and $2.3\%$ higher than the previous best performance.
This is significant since the previous best model has already utilized the execution-guided decoding.
In short, \ourexp achieves a new state-of-the-art result on the well-known benchmark \wikisql.

\begin{table*}[tb]
\small
\centering
\begin{tabular}{llllll} 
\toprule
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{l}{\textbf{Dev}} & \multicolumn{1}{l}{\textbf{Test}} & \textbf{Test\textsubscript{simple}} & \textbf{Test\textsubscript{complex}} & \textbf{Test\textsubscript{small}}  \\ 
\midrule
\multicolumn{6}{c}{\textit{Pre-trained Language Models}} \\
\multicolumn{1}{l}{\citet{chen2019tabfact}}  & $66.1$  & $65.1$ & $79.1$ &  $58.2$ & $68.1$      \\ 
\multicolumn{1}{l}{\citet{zhong-etal-2020-logicalfactchecker}}  & $71.8$ & $71.7$ & $85.4$ & $65.1$ & $74.3$\\
\multicolumn{1}{l}{\citet{shi-etal-2020-learn}}  & $72.5$ & $72.3$ & $85.9$ & $65.7$ & $74.2$\\
\multicolumn{1}{l}{\citet{zhang-etal-2020-table}} & $73.3$ & $73.2$ & $85.5$ & $67.2$ & ~~{--} \\
\multicolumn{1}{l}{\citet{yang-etal-2020-program}} & $74.9$ & $74.4$ & $88.3$ & $67.6$ & $76.2$ \\
\multicolumn{1}{l}{\citet{eisenschlos-etal-2020-understanding}}  & $81.0$ & $81.0$ & $92.3$ & $75.6$ & $83.9$ \\
\midrule
BART & $81.2$ & $80.8$ & $90.7$ & $76.0$ & $82.5$ \\
\ours & $\mathbf{84.6}$ & $\mathbf{84.2}$ & $\mathbf{93.9}$ & $\mathbf{79.6}$ & $\mathbf{85.9}$ \\
\midrule
\multicolumn{1}{l}{Human Performance}              &  -                      &      -  &  - & -      & $92.1$ \\
\bottomrule
\end{tabular}
\caption{Accuracies on \tabfact, including the Human Performance.}
\label{tab:tabfact_results}
\end{table*}

\textbf{\wtq}\;\;
On the more challenging \wtq, \ours also achieves a new state-of-the-art denotation accuracy of $57.5\%$, surpassing the previous best system by $4.8\%$ (\reftab{tab:wtq_results}).
Meanwhile, we find that BART alone can only reach the denotation accuracy of $38.0\%$, much worse than the performance of previous pre-training models.
We conjecture that the performance degradation could be attributed to the relatively small amount of training data in \wtq, which makes the adaptation of BART to tabular structures more challenging.
However, \ours delivers a dramatic improvement of $19.5\%$ over BART, indicating that in the low data regime, the improvements introduced by \ours are often more significant.

\textbf{SQA}\;\;
\reftab{tab:sqa_results} presents the performance of various models on the test set of \sqa, where \ours again obtains a new state-of-the-art denotation accuracy in terms of both the conversation level ($48.4\%$) and the sentence level ($74.5\%$).
This improvement is also a surprise to us since \sqa is a conversational dataset while our pre-training task is context-free.
Meanwhile, the substantial improvements of \ours over BART on \sqa continues to verify the same observation that \ours alleviates the low resource issue.

\textbf{\tabfact}\;\;
Beyond TableQA, \ourexp also excels at TableFV.
As shown in~\reftab{tab:tabfact_results}, \ours achieves new state-of-the-art results on all subsets of \tabfact.
For example, it surpasses the previous best system by $4.0\%$ on ${\rm Test}_{\rm complex}$.
The result shows that \ours endows BART with generic table understanding capabilities, which could be adapted to different downstream tasks, regardless of whether these tasks are highly similar to the \ourexp pre-training task or not.

\textbf{Overall Results}\;\;
Experimental results on four datasets show that \ourexp can broadly improve the model ability on understanding tables, especially in the low data regime.

\subsection{Multi-task Results}

As discussed in~\refsec{sec:getar}, our approach can easily perform multi-task learning, thereby conferring benefits to downstream tasks.
To verify it, we conducted multi-task fine-tuning experiments and obtained the following findings:
(1) when initialized by BART, multi-task fine-tuning boosts the performance of the target task significantly;
(2) when initialized by \ours, the gain of multi-task fine-tuning tends to be marginal, suggesting that most of the ``skills'' (loosely speaking) gained by multi-task learning can be acquired by our table pre-training.
Detailed results can be found in~\refapp{appendix:multi_task}.

==> Camera-Ready-ICLR 2022-Tapex/6_analysis.tex <==
\section{Analysis}

In this section, we carefully analyze our approach in terms of various aspects. Besides, we perform an exploratory analysis to provide more insights for future work, which can be found in~\refapp{appendix:exploratory}.

\textbf{SQL Execution by Pre-training}\;\;
In order to understand how well \ours performs SQL execution after pre-training, we analyze its performance on nearly $20,000$ held-out SQL queries over unseen tables.
Overall, the SQL execution accuracy is relatively high, as \ours correctly ``executes'' $89.6\%$ of the SQL queries\footnote{The full analysis about SQL execution can be found in~\refapp{appendix:sql}.}.
In particular, \ours performs better on {\texttt{\small Filter}}, {\texttt{\small Aggregate}} and {\texttt{\small Superlative}} operators, indicating that it is highly accurate in table cell selection and table aggregating.
Regarding {\texttt{\small Arithmetic}} and {\texttt{\small Comparative}} operators, \ours also does a good job, demonstrating its numerical reasoning skill on tables.
To summarize, \ourexp has learned to be a neural SQL executor with good selection, aggregating and numerical capabilities.

\begin{figure}[t!]
    \small
    \centering
    {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.85\textwidth}{\colorbox{red!14.970936}{\strut Who} \colorbox{red!13.802228}{\strut are} \colorbox{red!9.717735}{\strut the} \colorbox{red!6.521768}{\strut only} \colorbox{red!12.306012800000001}{\strut players} \colorbox{red!6.903509}{\strut listed} \colorbox{red!7.086827999999999}{\strut that} \colorbox{red!8.5836988}{\strut played} \colorbox{red!5.565175999999999}{\strut in} \colorbox{red!3.8364928}{\strut 2011} \colorbox{red!12.1032894}{\strut ?} \colorbox{red!9.142228999999999}{\strut [HEAD]} \colorbox{red!34.7230372}{\strut player} \colorbox{red!2.3756811}{\strut $|$} \colorbox{red!2.3478372000000003}{\strut year} \colorbox{red!2.7668154}{\strut $|$} \colorbox{red!5.4725796}{\strut round} \colorbox{red!2.8656236}{\strut $|$} \colorbox{red!3.826232}{\strut result} \colorbox{red!2.804299}{\strut $|$} \colorbox{red!5.366216799999999}{\strut opponent} \colorbox{red!2.9017952000000005}{\strut [ROW]} \colorbox{red!2.8313821999999997}{\strut 1} \colorbox{red!10.299296}{\strut ray} \colorbox{red!10.579882}{\strut mond} \colorbox{red!8.221680000000001}{\strut van} \colorbox{red!9.008807}{\strut bar} \colorbox{red!7.4133814}{\strut ne} \colorbox{red!6.2307126}{\strut ve} \colorbox{red!9.183715000000001}{\strut ld} \colorbox{red!3.4074528}{\strut $|$} \colorbox{red!3.1364577999999996}{\strut 2009} \colorbox{red!3.0261772}{\strut $|$} \colorbox{red!7.1568668}{\strut quarter} \colorbox{red!10.29556}{\strut -} \colorbox{red!7.359226}{\strut final} \colorbox{red!2.7560094}{\strut $|$} \colorbox{red!6.2080400000000004}{\strut won} \colorbox{red!3.2449352}{\strut $|$} \colorbox{red!8.8993174}{\strut j} \colorbox{red!10.114287200000001}{\strut elle} \colorbox{red!6.2276626}{\strut k} \colorbox{red!8.8740266}{\strut la} \colorbox{red!9.735318}{\strut as} \colorbox{red!7.475064000000001}{\strut en} \colorbox{red!3.1987599999999996}{\strut [ROW]} \colorbox{red!3.2400194}{\strut 2} \colorbox{red!9.723582799999999}{\strut ray} \colorbox{red!9.352703}{\strut mond} \colorbox{red!7.594534}{\strut van} \colorbox{red!8.3187848}{\strut bar} \colorbox{red!7.1613126}{\strut ne} \colorbox{red!6.573388}{\strut ve} \colorbox{red!9.092343999999999}{\strut ld} \colorbox{red!3.7991596000000003}{\strut $|$} \colorbox{red!3.5757356000000002}{\strut 2010} \colorbox{red!4.040925}{\strut $|$} \colorbox{red!8.162047999999999}{\strut 2} \colorbox{red!9.4804764}{\strut nd} \colorbox{red!8.9249826}{\strut round} \colorbox{red!3.7699683999999998}{\strut $|$} \colorbox{red!8.1906486}{\strut won} \colorbox{red!4.8999714}{\strut $|$} \colorbox{red!11.6535628}{\strut bre} \colorbox{red!13.612498}{\strut nd} \colorbox{red!12.360156}{\strut an} \colorbox{red!10.665865}{\strut d} \colorbox{red!12.203512000000002}{\strut olan} \colorbox{red!37.615702}{\strut [ROW]} \colorbox{red!42.653722}{\strut 3} \colorbox{red!55.65368000000001}{\strut ad} \colorbox{red!57.33528}{\strut rian} \colorbox{red!60.769768}{\strut le} \colorbox{red!61.41157200000001}{\strut w} \colorbox{red!61.32967}{\strut is} \colorbox{red!45.39855000000001}{\strut $|$} \colorbox{red!23.587676000000002}{\strut 2011} \colorbox{red!45.02534}{\strut $|$} \colorbox{red!40.120506}{\strut final} \colorbox{red!37.421062}{\strut $|$} \colorbox{red!33.088660000000004}{\strut won} \colorbox{red!38.722848}{\strut $|$} \colorbox{red!37.43384}{\strut g} \colorbox{red!38.099266}{\strut ary} \colorbox{red!21.687636}{\strut and} \colorbox{red!26.274652}{\strut erson} }}}
    \caption{The visualization results of attention weights from other tokens to the cell ``adrian lewis''. Intuitively, the darker the color, the more closely the word is associated with ``adrian lewis''. }
    \label{fig:table_understanding}
\end{figure}

\textbf{Table Understanding by Pre-training}\;\;
To provide insight on if \ours helps downstream tasks understand tables better, we visualize and analyze the self-attention of \ours (without fine-tuning) on sampled \wtq examples.
As shown in~\reffig{fig:table_understanding}, \ours seems to focus more on the row and the header where a cell corresponds to.
Taking the example from~\reffig{fig:table_understanding}, the attention weights imply that ``adrian lewis'' is closely associated with the first column ``player'' and the entire third row, which are the positions of ``adrian lewis'' in the structured table.

\begin{table*}[t!]
\centering
\small
\begin{tabular}{c p{5.1cm} m{1.3cm} m{2.3cm}}
\toprule
 \bf Operator & \bf Example Question & \bf BART & \bf \ours \\
\midrule
{\color{NavyBlue} \bf Select} &  What is {\color{NavyBlue} \bf the years won} for each team? &  $41.3$\% & $64.8\%$ (+$23.5$\%) \\
{\color{Orange} \bf Filter} & How long did {\color{Orange} \bf Taiki Tsuchiya} last?  &  $40.1$\% & $65.7$\% (+$25.6$\%) \\ 
{\color{Bittersweet} \bf Aggregate} & What is the {\color{Bittersweet} \bf amount of} matches drawn?
 & $26.9$ \% & $57.4$\% (+$30.5$\%) \\
{\color{Green} \bf Superlative} & What was the {\color{Green} \bf last} Baekje Temple? & $46.3$ \% & $64.3$\% (+$18.0$\%) \\ 
{\color{Cyan} \bf Arithmetic} & What is the {\color{Cyan} \bf difference} between White voters and Black voters in 1948? & $33.1$ \% & $53.5$\% (+$20.4$\%) \\ 
{\color{Plum} \bf Comparative} & Besides Tiger Woods, what other player won {\color{Plum} \bf between 2007 and 2009}? & $30.0$ \% & $55.9$\% (+$25.9$\%) \\ 
{\color{BlueViolet} \bf Group} & What was score {\color{BlueViolet} \bf for each} winning game? & $49.5$ \% & $66.7$\% (+$17.2$\%) \\
\bottomrule
\end{tabular}
\caption{The most common operators in the randomly selected $500$ questions from \wtq dev set. Listed are, the operator, the example question with the operator semantic (i.e., the {\color{NavyBlue} \bf colorful} spans), the performance of BART and \ours on the operator.}
\label{table:operators}
\end{table*}

\textbf{Table Reasoning by Pre-training}\;\;
To understand if \ours can improve table reasoning, we compare the performance of \ours to BART on $500$ randomly selected questions and manually analyzed them in~\reftab{table:operators}.
One can find that \ours significantly boosts the performance on all operators, implying that it does enhance BART's capabilities for joint reasoning over text and tables.

\textbf{The Scale of Pre-training Corpus}\;\;
\reffig{fig:analysis_scale} illustrates downstream performance with different scales of the pre-training corpus.
It can be seen that even if our pre-training corpus is synthetic, scaling up the pre-training corpus generally brings positive effects.
The observation is analogous to the one in language modeling \citep{NEURIPS2020_1457c0d6}: the larger the pre-training corpus, the better the downstream performance.
By the comparison across different datasets, we can find that for simple tasks like \wikisql, the gains by scaling up pre-training corpus become marginal, while they remain non-trivial for complex tasks like \tabfact.
Meanwhile, both downstream datasets in the low data regime show a positive trend by increasing the pre-training corpus.
Conclusively, the scale matters when the downstream task is difficult, or the downstream dataset is relatively small.

\input{figures/pretrain_scale}

\textbf{The Efficiency of Pre-training}\;\;
As mentioned in~\refsec{sec:intro}, the pre-training efficiency of existing table pre-training approaches is relatively low, as they usually require an extremely large corpus.
Therefore, taking \wtq as an example, we compare the pre-training efficiency of \ours with \tapas~\citep{herzig-etal-2020-tapas}, \tabert~\citep{yin-etal-2020-tabert} and \textsc{GraPPa}~\citep{Yu2020GraPPaGP}.
It is worth noting that part of the pre-training corpus for \textsc{GraPPa} comes from human-annotated, high-quality parallel data.
As shown in~\reffig{fig:flops_intro}, \ours can yield very promising performance when using a much smaller pre-training corpus, indicating that our proposed SQL execution pre-training task is more efficient than other table pre-training tasks.

\textbf{Limitations}\;\;
The first limitation of our approach is that it cannot ideally handle large tables.
As mentioned above, we employ the table flattening technique to represent a table.
It works well when the table is relatively small, but it becomes infeasible when the table is too large to fit in memory.
In practice, we can compress tables by removing some unrelated rows or columns, which would decrease downstream performance.
The second limitation is that the task of text-to-SQL cannot benefit from our proposed table pre-training.
We have tried to apply \ours for a text-to-SQL task, where the input remains the same and the output converts to SQL.
However, \ours does not show a significant advantage over BART.
We attribute this to two factors:
first, our synthetic pre-training corpus does not contribute to grounding, one of the most important factors for semantic parsing \citep{qian2021awakening};
second, table reasoning capabilities (e.g., aggregate) learned by \ours may not be necessary for SQL generation.
For example, a model could still understand an NL phrase ``total'' as the aggregation function ``sum'', even though it is unaware of the mathematical meaning of ``sum''.
% Both of these are our future work to extend \ourexp.



==> Camera-Ready-ICLR 2022-Tapex/7_related_work.tex <==

\section{Related Work}\label{sec:related}

\textbf{Table Pre-training}\;\;
The work most related to ours is table pre-training whose key factors include the pre-training corpus and the pre-training task.
As for the pre-training corpus, most of previous works almost collect NL-table data to perform table pre-training.
They either mined a large corpus of tables and their NL sentence contexts \citep{yin-etal-2020-tabert,herzig-etal-2020-tapas}, leveraged human-annotated parallel NL-table datasets for pre-training \citep{deng-etal-2021-structure,Yu2020GraPPaGP}, or synthesized a NL-table corpus using human-written templates \citep{Yu2020GraPPaGP,eisenschlos-etal-2020-understanding}.
Our work is different from theirs because we are the first to use pure synthetic SQL-table data for table pre-training, which allows us to automatically synthesize a diverse, large-scale, and high-quality pre-training corpus.
As for the pre-training task, existing works proposed several pre-training tasks, such as Mask Column Prediction \citep{yin-etal-2020-tabert}, Multi-choice Cloze at the Cell Level \citep{wang2021tuta} and Structure Grounding \citep{deng-etal-2021-structure}.
Different from all of them, we present a novel SQL execution task to perform table pre-training.

\textbf{Joint Understanding on Table and Text}\;\;
As our experiments are mainly on TableQA and TableFV, our work is also closely related to previous methods for these tasks.
For TableQA, previous works almost formulate it as a weakly semantic parsing task \citep{liang18mapo,wang19wikitable,guo-etal-2021-weakly-supervised}, which always employ reinforcement learning to optimize semantic parsers over tables.
Although these parsers produce logic forms (e.g., SQL), they have difficulties in training due to the large search space and the presence of spurious programs \citep{goldman-etal-2018-weakly}.
In addition, another promising line of work has emerged in recent advances \citep{mueller-etal-2019-answering,herzig-etal-2020-tapas}, which aims at answering NL sentences without logical forms.
This line of work predicts answer(s) by selecting cell values and optionally applying an aggregation operator to them.
They can be easily trained, but their modeling ability is limited.
For example, it is hard to support compound aggregation operators such as \texttt{\small max(Year) - min(Year)}.
What makes our approach different from these works is that we employ generative models to handle TableQA and can enjoy the end-to-end training and flexibility simultaneously.
For TableFV, previous works usually employ specialized architectures with limited scalability \citep{shi-etal-2020-learn, yang-etal-2020-program,shi-etal-2021-logic}.
For example, \citet{zhong-etal-2020-logicalfactchecker} leveraged a graph construction mechanism, a semantic parser, and a semantic composition model to capture the connections among the NL sentence and the table.
While the approach works well for TableFV, it is not easily applied to other table-related tasks.
Compared with them, our approach works well for a variety of downstream tasks in the same architecture.


==> Camera-Ready-ICLR 2022-Tapex/8_conclusion.tex <==

\section{Conclusion}

In this paper, we present \ours, an execution-centric table pre-training approach whose corpus is automatically synthesized via sampling SQL queries and their execution results.
\ours addresses the data scarcity challenge in table pre-training by learning a neural SQL executor on a diverse, large-scale, and high-quality synthetic corpus.
Experimental results on four downstream datasets demonstrate that \ours outperforms previous table pre-training approaches by a large margin and achieves new state-of-the-art results on all of them.
Our work opens the way to exploit structured data by pre-training on synthetic executable programs, which is conceptually simple and has great potential to be extended to other research areas (e.g., knowledge base).

\section*{Acknowledgement}

We would like to thank all the anonymous reviewers for their constructive feedback.
The first author Qian is supported by the Academic Excellence Foundation of Beihang University for PhD Students.


==> Camera-Ready-ICLR 2022-Tapex/figures/complex.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
    Difficulty & wtq & sqa & tabfact & wiki \\
    BART & 37.2 & 58.6 & 81.2 & 87.3 \\
    $\leq$ Easy & 41.5 & 61.4 & 81.1 & 86.9 \\
    $\leq$ Medium   & 52.1 & 67.6 & 83.5 & 87.7 \\
    $\leq$ Hard   & 53.9 & 68.1 & 83.8 & 88.1 \\
    $\leq$ Extra Hard & 54.2 & 68.9 & 83.6  & 88.8 \\
}\complexdata

\pgfplotsset{every axis/.append style={
                    label style={font=\large},
                    tick label style={font=\large} 
                    }}
\begin{figure}[hbt]
    \centering
    \begin{tikzpicture}[scale=0.8]
        \begin{axis}[
                ybar=5pt,
                bar width=.33cm,
                enlarge x limits=0.2,
                width=1.1\textwidth,
                height=.4\textwidth,
                legend style={at={(0.5,1.20)},
                anchor=north,legend columns=-1},
                symbolic x coords={BART, $\leq$ Easy, $\leq$ Medium, $\leq$ Hard, $\leq$ Extra Hard},
                xtick=data,
                nodes near coords,
                every node near coord/.append style={font=\small},
                nodes near coords align={vertical},
                ymin=30,ymax=100,
                ylabel={Task Performance (\%)},
                % xlabel={Amount of Pretraining Corpus (Millions)}
            ]
            \addplot table[x=Difficulty,y=wtq]{\complexdata};
            \addplot table[x=Difficulty,y=sqa]{\complexdata};
            \addplot table[x=Difficulty,y=tabfact]{\complexdata};
            \addplot table[x=Difficulty,y=wiki]{\complexdata};
            \legend{\wtq, \sqa, \tabfact, \wikisql}
        \end{axis}
    \end{tikzpicture}
    \caption{The performance of downstream tasks (dev sets) at different pre-training difficulties with the same amount of examples ($0.5$ Million). $\leq$\,Medium means that we only use SQL query templates with a difficulty level less than or equal to Medium when synthesizing its pre-training corpus. Notably, $\leq$\,Extra Hard is equivalent to using all SQL query templates.}
    \label{fig:analysis_diff}
\end{figure}

==> Camera-Ready-ICLR 2022-Tapex/figures/flops_intro.tex <==
% \begin{figure}[t!]
%     \centering
%         \begin{tikzpicture}[scale=0.4]
%         \begin{axis}[
%             legend style={nodes={scale=1.0, transform shape}},
%             % title={Overall Schema Linking Recall},
%             xlabel={Amount of Pretraining Corpus (Millions)},
%             xtick pos=left,
%             xmode=log,
%             log ticks with fixed point,
%             ylabel={\wtq Denotation Accuracy (\%)},
%             xmin=0.005, xmax=100.0,
%             ymin=0.33, ymax=0.6,
%             xtick={0.01, 0.1, 1.0, 10.0, 100.0},
%             xticklabels={$10^{-2}$, $10^{-1}$, $10^0$, $10^1$, $10^2$},
%             ytick={0.35, 0.4, 0.45, 0.5, 0.55, 0.6},
%             yticklabels={$35.0$, $40.0$,$45.0$,$50.0$,$55.0$,$60.0$},
%             % ytick={0.3,0.5,0.7,0.9,1.0},
%             legend pos=south east,
%             ymajorgrids=true,
%             grid style=dashed
%         ]
         
%         \addplot[
%             color=purple,
%             dotted,
%             mark options={solid},
%             mark=*,
%             line width=1.5pt,
%             mark size=2pt
%             ]
%             coordinates {
%             (0.01, 0.380)
%             (0.1, 0.486)
%             (0.5, 0.542)
%             (1.0, 0.561)
%             (3.0, 0.570)
%             (5.0, 0.570)
%             };            
%             \addlegendentry{\ours}

%         \addplot[
%             color=gray,
%             mark=square*,
%             mark options={solid},
%             mark size=3pt
%             ]
%             coordinates {
%             % BART
%             (0.007, 0.372)
%         };
%         \addplot[
%             color=black,
%             mark=pentagon*,
%             mark options={solid},
%             mark size=3pt
%             ]
%             coordinates {
%             % GraPPa
%             (0.867, 0.519)
%             };
%         \addplot[
%             color=brown,
%             mark=triangle*,
%             mark options={solid},
%             mark size=4pt
%             ]
%             coordinates {
%             % TaPaS
%             (21.3, 0.488)
%             };
%         \addplot[
%             color=blue,
%             mark=diamond*,
%             mark options={solid},
%             mark size=4pt
%             ]
%             coordinates {
%             % TaBERT
%             (26.3, 0.530)
%             };
%         \node at (axis cs:0.012, 0.357){BART};
%         \node at (axis cs:1.2, 0.504){\textsc{GraPPa}};
%         \node at (axis cs:21.3, 0.473){\textsc{TaPaS}};
%         \node at (axis cs:26.3, 0.510){\textsc{TaBERT}};
%         \end{axis}
%         \end{tikzpicture}
%     \caption{The amount of pre-training corpus vs. \wtq dev set denotation accuracy. \ours surpasses existing table pre-training approaches with a much smaller corpus, demonstrating its high efficiency.}
%     % Note that \textsc{GraPPa} \cite{Yu2020GraPPaGP} collects human annotated parallel data for table pre-training.
%     \label{fig:flops_intro}
% \end{figure}


==> Camera-Ready-ICLR 2022-Tapex/figures/pretrain_scale.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
    Scale & wtq & sqa & tabfact & wiki \\
    $0.1$   & 48.6 & 65.3 & 82.8 & 88.1 \\
    $0.5$   & 54.2 & 68.9 & 83.6  & 88.8\\
    $1.0$   & 56.1 & 70.2 & 83.8  & 89.2 \\
    $5.0$  & 57.0 & 70.3  & 84.6  & 89.1 \\
    }\mydata

\pgfplotsset{every axis/.append style={
                    label style={font=\large},
                    tick label style={font=\large} 
                    }}
\begin{figure}[t!]
    \begin{minipage}{0.53\linewidth}
    \centering
    \begin{tikzpicture}[scale=0.7]
        \begin{axis}[
                ybar=5pt,
                bar width=.33cm,
                enlarge x limits=0.2,
                width=1.4\textwidth,
                height=.7\textwidth,
                legend style={at={(0.5,1.20)},
                anchor=north,legend columns=-1},
                symbolic x coords={$0.1$, $0.5$, $1.0$, $5.0$},
                xtick=data,
                nodes near coords,
                every node near coord/.append style={font=\small},
                nodes near coords align={vertical},
                ymin=40,ymax=100,
                ylabel={Task Performance (\%)},
                xlabel={Amount of Pretraining Corpus (Millions)}
            ]
            \addplot table[x=Scale,y=wtq]{\mydata};
            \addplot table[x=Scale,y=sqa]{\mydata};
            \addplot table[x=Scale,y=tabfact]{\mydata};
            \addplot table[x=Scale,y=wiki]{\mydata};
            \legend{\wtq, \sqa, \tabfact, \wikisql}
        \end{axis}
    \end{tikzpicture}
    \caption{The illustration of downstream tasks performance with different scales of pre-training corpus. Scaling up the pre-training corpus of \ours generally brings positive effects across datasets.}
    \label{fig:analysis_scale}
    \end{minipage}
    \hspace{0.1cm}
    \begin{minipage}{0.46\linewidth}
    \centering
            \begin{tikzpicture}[scale=0.57]
                \begin{axis}[
                    legend style={nodes={scale=1.0, transform shape}},
                    xlabel={Amount of Pretraining Corpus (Millions)},
                    xtick pos=left,
                    xmode=log,
                    log ticks with fixed point,
                    ylabel={Denotation Accuracy (\%)},
                    xmin=0.005, xmax=100.0,
                    ymin=0.33, ymax=0.6,
                    xtick={0.01, 0.1, 1.0, 10.0, 100.0},
                    xticklabels={$10^{-2}$, $10^{-1}$, $10^0$, $10^1$, $10^2$},
                    ytick={0.35, 0.4, 0.45, 0.5, 0.55, 0.6},
                    yticklabels={$35.0$, $40.0$,$45.0$,$50.0$,$55.0$,$60.0$},
                    legend pos=south east,
                    ymajorgrids=true,
                    grid style=dashed
                ]
                 
                \addplot[
                    color=purple,
                    dotted,
                    mark options={solid},
                    mark=*,
                    line width=1.5pt,
                    mark size=2pt
                    ]
                    coordinates {
                    (0.01, 0.380)
                    (0.1, 0.486)
                    (0.5, 0.542)
                    (1.0, 0.561)
                    (3.0, 0.570)
                    (5.0, 0.570)
                    };            
                    \addlegendentry{\ours}
        
                \addplot[
                    color=gray,
                    mark=square*,
                    mark options={solid},
                    mark size=3pt
                    ]
                    coordinates {
                    (0.007, 0.372)
                };
                \addplot[
                    color=black,
                    mark=pentagon*,
                    mark options={solid},
                    mark size=3pt
                    ]
                    coordinates {
                    (0.867, 0.519)
                    };
                \addplot[
                    color=brown,
                    mark=triangle*,
                    mark options={solid},
                    mark size=4pt
                    ]
                    coordinates {
                    (21.3, 0.488)
                    };
                \addplot[
                    color=blue,
                    mark=diamond*,
                    mark options={solid},
                    mark size=4pt
                    ]
                    coordinates {
                    (26.3, 0.530)
                    };
                \node at (axis cs:0.012, 0.357){BART};
                \node at (axis cs:1.2, 0.504){\textsc{GraPPa}};
                \node at (axis cs:21.3, 0.473){\textsc{TaPaS}};
                \node at (axis cs:26.3, 0.510){\textsc{TaBERT}};
                \end{axis}
                \end{tikzpicture}
            \caption{The amount of pre-training corpus vs. denotation accuracy on \wtq dev set. \ours surpasses existing table pre-training approaches with a much smaller corpus, showing its high efficiency.}
            \label{fig:flops_intro}
    \end{minipage}
\end{figure}

==> figures/flops_intro.tex <==
% \begin{figure}[t!]
%     \centering
%         \begin{tikzpicture}[scale=0.4]
%         \begin{axis}[
%             legend style={nodes={scale=1.0, transform shape}},
%             % title={Overall Schema Linking Recall},
%             xlabel={Amount of Pretraining Corpus (Millions)},
%             xtick pos=left,
%             xmode=log,
%             log ticks with fixed point,
%             ylabel={\wtq Denotation Accuracy (\%)},
%             xmin=0.005, xmax=100.0,
%             ymin=0.33, ymax=0.6,
%             xtick={0.01, 0.1, 1.0, 10.0, 100.0},
%             xticklabels={$10^{-2}$, $10^{-1}$, $10^0$, $10^1$, $10^2$},
%             ytick={0.35, 0.4, 0.45, 0.5, 0.55, 0.6},
%             yticklabels={$35.0$, $40.0$,$45.0$,$50.0$,$55.0$,$60.0$},
%             % ytick={0.3,0.5,0.7,0.9,1.0},
%             legend pos=south east,
%             ymajorgrids=true,
%             grid style=dashed
%         ]
         
%         \addplot[
%             color=purple,
%             dotted,
%             mark options={solid},
%             mark=*,
%             line width=1.5pt,
%             mark size=2pt
%             ]
%             coordinates {
%             (0.01, 0.380)
%             (0.1, 0.486)
%             (0.5, 0.542)
%             (1.0, 0.561)
%             (3.0, 0.570)
%             (5.0, 0.570)
%             };            
%             \addlegendentry{\ours}

%         \addplot[
%             color=gray,
%             mark=square*,
%             mark options={solid},
%             mark size=3pt
%             ]
%             coordinates {
%             % BART
%             (0.007, 0.372)
%         };
%         \addplot[
%             color=black,
%             mark=pentagon*,
%             mark options={solid},
%             mark size=3pt
%             ]
%             coordinates {
%             % GraPPa
%             (0.867, 0.519)
%             };
%         \addplot[
%             color=brown,
%             mark=triangle*,
%             mark options={solid},
%             mark size=4pt
%             ]
%             coordinates {
%             % TaPaS
%             (21.3, 0.488)
%             };
%         \addplot[
%             color=blue,
%             mark=diamond*,
%             mark options={solid},
%             mark size=4pt
%             ]
%             coordinates {
%             % TaBERT
%             (26.3, 0.530)
%             };
%         \node at (axis cs:0.012, 0.357){BART};
%         \node at (axis cs:1.2, 0.504){\textsc{GraPPa}};
%         \node at (axis cs:21.3, 0.473){\textsc{TaPaS}};
%         \node at (axis cs:26.3, 0.510){\textsc{TaBERT}};
%         \end{axis}
%         \end{tikzpicture}
%     \caption{The amount of pre-training corpus vs. \wtq dev set denotation accuracy. \ours surpasses existing table pre-training approaches with a much smaller corpus, demonstrating its high efficiency.}
%     % Note that \textsc{GraPPa} \cite{Yu2020GraPPaGP} collects human annotated parallel data for table pre-training.
%     \label{fig:flops_intro}
% \end{figure}

